Scalable Spider Nests (...Or How to Graphically Grok Transversal Non-Clifford Gates)

This is the second in a series of "graphical grokking" papers in which we study how stabiliser codes can be understood using the ZX-calculus. In this paper we show that certain complex rules involving ZX-diagrams, called spider nest identities, can be captured succinctly using the scalable ZX-calculus, and all such identities can be proved inductively from a single new rule using the Clifford ZX-calculus. This can be combined with the ZX picture of CSS codes, developed in the first "grokking" paper, to give a simple characterisation of the set of all transversal diagonal gates at the third level of the Clifford hierarchy implementable in an arbitrary CSS code.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{A. D\'iaz-Caro and V. Zamdzhiev (Eds.):\\
Quantum Physics and Logic 2024 (QPL 2024)\\
EPTCS 406, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.406.4}{10.4204/EPTCS.406.4}}
\pdfoutput=1


==> preamble.tex <==
\RequirePackage{etex}
\usepackage[T1]{fontenc}

% \renewcommand{\theenumi}{\arabic{enumi}.}
% \setcounter{tocdepth}{2}
% \setcounter{secnumdepth}{3}

% \usepackage{lmodern}

\usepackage{morewrites} % Prevent ``No room for a new \write'' error.

\usepackage[activate=true,
    final,
    tracking=true,
    % kerning=true,
    % spacing=true,
    factor=1100,
    stretch=10,
    shrink=10]{microtype}
\microtypecontext{spacing=nonfrench}

% \usepackage[hyphens]{url}
\usepackage{url}
\usepackage{hyperref}

% \hypersetup{
%      colorlinks = true,
%      linkcolor = blue!70!black,
%      anchorcolor = blue!70!black,
%      citecolor = red!70!black,
%      filecolor = blue!70!black,
%      urlcolor = blue!70!black
% }
\usepackage[hyphenbreaks]{breakurl}
\usepackage[all]{hypcap}

% \font\omding=omding

\usepackage{amsmath,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{xspace,enumerate,epsfig}
\usepackage{graphicx}
\graphicspath{{.}{./figures/}}
\usepackage{marvosym}
\usepackage{bm}
\usepackage{tabu}
\tabulinesep=2mm

%% enables using PDF figures in cache/, if they exist
% \usepackage[draft]{tikzit}
\usepackage{tikzit}

\input{circuits.tikzdefs}
\input{circuits.tikzstyles}

% \usepackage{stmaryrd}
\newcommand{\llbracket}{[\![}
\newcommand{\rrbracket}{]\!]}
\usepackage{keycommand}

\usepackage{ifthen}


% OURS
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem{example*}[theorem]{Example*}
\newtheorem{examples*}[theorem]{Examples*}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remark*}[theorem]{Remark*}
\newtheorem{question}[theorem]{Question}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{exer}[theorem]{Exercise}
\newtheorem{exer*}[theorem]{Exercise*}

% \newcommand{\TODOa}[1]{{\color{blue} [\textbf{TODO:} #1]}}
% \newcommand{\TODOj}[1]{{\color{green!50!black} [\textbf{TODO:} #1]}}
% \newcommand{\NOTEa}[1]{{\color{blue} [\textbf{a:} #1]}}
% \newcommand{\NOTEj}[1]{{\color{green!50!black} [\textbf{j:} #1]}}
\newcommand{\df}[1]{\textbf{#1}}

\hyphenation{line-break line-breaks docu-ment triangle cambridge amsthdoc
  cambridgemods baseline-skip author authors cambridgestyle en-vir-on-ment polar
  ortho-normal}






\newcommand{\bitpauli}[3]{\big(#1\,|\,#2\big)\,\textrm{\color{blue!50!gray}\small$\bm{#3}$ } }
\DeclarePairedDelimiter{\inn}{\langle}{\rangle}

%\newcommand{\lp}{\bm{0}}
%\newcommand{\lm}{\bm{2}}
%\newcommand{\lpi}{\bm{1}}
%\newcommand{\lmi}{\bm{3}}

\newcommand{\lp}{\texttt{\color{blue!50!gray}\small\textbf{+}}}
\newcommand{\lm}{\texttt{\color{blue!50!gray}\small\textbf{-}}}
\newcommand{\lpi}{\texttt{\color{blue!50!gray}\small\textbf{+$\bm{i}$}}}
\newcommand{\lmi}{\texttt{\color{blue!50!gray}\small\textbf{-$\bm{i}$}}}


\newcommand{\biggline}{\bigg|}
\DeclareMathOperator\Dom{Dom}
\DeclareMathOperator\Zer{Zer}
\DeclareMathOperator\Dim{Dim}
\DeclareMathOperator\diag{diag}
% \DeclareMathOperator\Re{Re}
% \DeclareMathOperator\Im{Im}

\setcounter{MaxMatrixCols}{20} % Needed if you want pmatrix with more than 10 columns

